Transformation-Interaction-Rational Representation for Symbolic Regression

Symbolic Regression searches for a function form that approximates a dataset often using Genetic Programming. Since there is usually no restriction to what form the function can have, Genetic Programming may return a hard to understand model due to non-linear function chaining or long expressions. A novel representation called Interaction-Transformation was recently proposed to alleviate this problem. In this representation, the function form is restricted to an affine combination of terms generated as the application of a single univariate function to the interaction of selected variables. This representation obtained competing solutions on standard benchmarks. Despite the initial success, a broader set of benchmarking functions revealed the limitations of the constrained representation. In this paper we propose an extension to this representation, called Transformation-Interaction-Rational representation that defines a new function form as the rational of two Interaction-Transformation functions. Additionally, the target variable can also be transformed with an univariate function. The main goal is to improve the approximation power while still constraining the overall complexity of the expression. We tested this representation with a standard Genetic Programming with crossover and mutation. The results show a great improvement when compared to its predecessor and a state-of-the-art performance for a large benchmark.

==> floats/texts/ITEA.tex <==
\SetKwInOut{Input}{Input}
\SetKwInOut{Output}{Output}

\Input{ Explanatory variables $\mathbf{X}$ and response variable $\mathbf{y}$}
\Output{ Symbolic function $\widehat{f}$}

\SetKwData{Pop}{pop}
\SetKwData{Filhos}{child}
\SetKwData{F}{f}
\SetKwData{Mt}{mt}
\SetKwData{Lb}{lb}
\SetKwData{Ub}{ub}
\SetKwData{Funs}{funs}
\SetKwData{P}{p}
\SetKwData{P'}{p'}
\SetKwData{MutElegiveis}{elegibleMut}


\SetKwFunction{SubsInter}{subsInter}
\SetKwFunction{Adicionar}{add}
\SetKwFunction{Remover}{drop}
\SetKwFunction{InterPos}{interPos}
\SetKwFunction{InterNeg}{interNeg}
\SetKwFunction{Pontuacao}{score}

\SetKwFunction{GerarPopAleatoria}{CreateRandomPop}
\SetKwFunction{RemoveTermosInvalidos}{RemoveInvalidTerms}
\SetKwFunction{Mutacao}{mutate}
\SetKwFunction{Selecao}{select}


\BlankLine

%\Pop $\leftarrow$ \GerarPopAleatoria{\Mt, \Lb, \Ub, \Funs}\;
\Pop $\leftarrow$ \GerarPopAleatoria{}\;
%\For{\P $\in$ \Pop}{
%    \P' $\leftarrow$ \RemoveTermosInvalidos{\P}\;
%    \Pop $\leftarrow$ \Pop $\setminus$ \{\P\}\;
%    \If{\P'.nTerms $\geq$ 1}{
%        \Pop $\leftarrow$ \Pop $\cup$ \{\P'\}\;
%    }
%}

\While{Stop criteria not met}{
    \Filhos $\leftarrow \varnothing$\;
    
    \For{\P $\in$ \Pop}{
        \MutElegiveis $\leftarrow$ \{\SubsInter\};
        
        \If{\P.nTerms $<$ \Mt}{
            \MutElegiveis $\leftarrow$ \MutElegiveis $\cup$ \{\Adicionar, \InterPos, \InterNeg\};
        }
        \If{\P.nTerms $>$ 1}{
            \MutElegiveis $\leftarrow$ \MutElegiveis $\cup$ \{\Remover\};
        }
        
        \F $\leftarrow$ \Mutacao{\P, \MutElegiveis}\;
        \F $\leftarrow$ \RemoveTermosInvalidos{\F}\;
        \If{\F.nTerms $\geq$ 1}{
            \Filhos $\leftarrow$ \Filhos $\cup$ \{\F\}\;
        }
    }
    
    \Pop $\leftarrow$ \Selecao{\Pop $\cup$ \Filhos}\;
}

\Return $arg \max $ \{\Pontuacao(\P) for \P $\in$ \Pop\}\;


==> floats/texts/Parameters.tex <==
\begin{tabular}{@{}ll@{}}
\toprule\midrule
Algorithm & Parameters \\ \midrule
ITEA & \begin{tabular}[c]{@{}l@{}}population = $300$\\ generations = 300\\ strength range = $(-5, 5)$\\ max terms = $15$\\ funs = $\{id, sin, cos, tanh, \sqrt{}, exp, log, exp(-\cdot), arcsin\}$ \end{tabular} \\\midrule
XGB & \begin{tabular}[c]{@{}l@{}}max depth = $[2, 3, 5]$\\ n estimators = $[100, 1000]$\\ learning rate = $[1e-5, 1e-3, 1e-1]$\\ min samples split = $[0.02, 0.05, 0.1]$\end{tabular} \\\midrule
RF & \begin{tabular}[c]{@{}l@{}}n estimators = $[10, 100, 1000]$\\ min samples split = $[0.02, 0.05, 0.10]$\end{tabular} \\ \midrule
KR & \begin{tabular}[c]{@{}l@{}}alpha = $[2, 3, 5]$\\ kernel = $[chi2, linear, poly, rbf]$\\ gamma = $[1e-5, 1e-3, 1e-1]$, \\ degree = $5$\end{tabular} \\\midrule\bottomrule
\end{tabular}

==> floats/texts/TreeExample.tex <==
\begin{tikzpicture}[
    level 1/.style={sibling distance=5.5em, level distance=.75cm},
    level 2/.style={sibling distance=5em}
]
    \node[circle,draw]{$\cdot$}
    	child{ node[circle,draw]{$q$} }
    	child{ node[circle,draw]{$+$}
        	child{ node[circle,draw] {$E_f$}}
        	child{ node[circle,draw]{$\cdot$}
            	child{ node[circle,draw]{$B$} }
            	child{ node[circle,draw]{$\cdot$}
                	child{ node[circle,draw]{$v$} }
                	child{ node[circle,draw]{$sin$}
                	    child{ node[circle,draw]{$\theta$} }
                	}
                }
            }
    	};
\end{tikzpicture}

==> floats/texts/equationsBarplots.tex <==
\begin{tabular}{@{}lcc@{}}
\toprule\midrule
 & 5 Best & 5 Worst \\ \midrule
\multirow{5}{*}{Global} & $e^{(-theta^2/2)}/\sqrt{2 \cdot \pi}$ & $p_d/(4 \cdot \pi \cdot \epsilon) \cdot 3 \cdot z/r^5 \cdot \sqrt{x^2+y^2}$ \\ \cmidrule(l){2-3} 
 & $m_0/\sqrt(1-v^2/c^2)$ & $x1 \cdot (cos(\omega \cdot t)+\alpha \cdot cos(\omega \cdot t)^2)$ \\ \cmidrule(l){2-3} 
 & $mu \cdot Nn$ & $Int_0 \cdot sin(n \cdot \theta/2)^2/sin(\theta/2)^2$ \\ \cmidrule(l){2-3} 
 & $q1 \cdot r/(4 \cdot \pi \cdot \epsilon \cdot r^3)$ & $sin(E_n \cdot t/(h/(2 \cdot \pi)))^2$ \\ \cmidrule(l){2-3} 
 & $q2 \cdot Ef$ & $q \cdot (Ef+B \cdot v \cdot sin(\theta))$ \\ \midrule
\multirow{5}{*}{Local} & $e^{(-theta^2/2)}/\sqrt{2 \cdot \pi}$ & $p_d/(4 \cdot \pi \cdot \epsilon) \cdot 3 \cdot z/r^5 \cdot \sqrt{x^2+y^2}$ \\ \cmidrule(l){2-3} 
 &$m_0/\sqrt(1-v^2/c^2)$ & $\frac{G \cdot m1 \cdot m2}{(x2-x1)^2+(y2-y1)^2+(z2-z1)^2}$ \\ \cmidrule(l){2-3} 
 & $mu \cdot Nn$ & $x1 \cdot (cos(\omega \cdot t)+\alpha \cdot cos(\omega \cdot t)^2)$ \\ \cmidrule(l){2-3} 
 & $q1 \cdot r/(4 \cdot pi \cdot \epsilon \cdot r^3)$ & $q \cdot (Ef+B \cdot v \cdot sin(\theta))$ \\ \cmidrule(l){2-3} 
 & $q2 \cdot Ef$ & $sqrt((x2-x1)^2+(y2-y1)^2)$ \\ \midrule\bottomrule 
\end{tabular}

==> floats/texts/meanTime.tex <==
\iffalse
% Sem desvios padrões e com 3 casas decimais (truncamento)
\begin{tabular}{@{}llllll@{}}
\toprule
 & Train & SHAP & LIME & ELI5 & ME \\ \midrule
ITEA & $108.162$ & $9.756$ & $358.230$ & $0.013$ & $0.456$ \\
XGB & $0.025$ & $5.624$ & $335.811$ & $0.011$ & - \\
RF & $0.067$ & $7.523$ & $318.691$ & $0.096$ & - \\ \bottomrule
\end{tabular}
\fi 

% Com desvios padrões e duas casas decimais (arredondamento) (transposta da primeira)
\begin{tabular}{lccc}
\toprule \midrule
       & ITEA                & XGB                 & RF                  \\ \midrule
Train  & $108.36 \pm 33.65$  & $0.02 \pm 0.00$     & $0.06 \pm 0.01$     \\
SHAP   & $9.79 \pm 13.61$    & $5.64 \pm 6.74$     & $7.55 \pm 6.85$     \\
LIME   & $358.47 \pm 123.14$ & $336.40 \pm 112.87$ & $319.35 \pm 101.49$ \\
%ELI5   & $0.01 \pm 0.01$     & $0.01 \pm 0.00$     & $0.10 \pm 0.03$     \\
PE     & $0.46 \pm 0.24$     & -                   & -                   \\ \midrule \bottomrule
\end{tabular}

==> floats/texts/statisticalTests/absmax/stats-gradient-global-AbsMax.tex <==
\begin{tabular}{rllllllll}
\toprule \midrule
 & LIME-ITEA & LIME-KR & LIME-RF & LIME-XGB & PE-ITEA & SHAP\_adj-ITEA & SHAP\_adj-KR & SHAP\_adj-RF \\ \hline
   LIME-KR & 1.0e+00 &  &  &  &  &  &  &  \\ 
   LIME-RF & 7.1e-02 & 1.2e-02* &  &  &  &  &  &  \\ 
   LIME-XGB & 1.0e+00 & 1.0e+00 & 1.0e+00 &  &  &  &  &  \\ 
   PE-ITEA & 1.2e-21*** & 2.1e-21*** & 6.2e-24*** & 1.5e-22*** &  &  &  &  \\ 
   SHAP\_adj-ITEA & 5.9e-03** & 8.7e-02 & 6.6e-08*** & 9.5e-05*** & 1.6e-18*** &  &  &  \\ 
   SHAP\_adj-KR & 8.0e-02 & 5.5e-01 & 6.0e-07*** & 8.5e-04*** & 7.1e-19*** & 1.0e+00 &  &  \\ 
   SHAP\_adj-RF & 6.3e-01 & 1.7e-01 & 1.0e+00 & 1.0e+00 & 3.3e-23*** & 6.1e-06*** & 3.1e-05*** &  \\ 
   SHAP\_adj-XGB & 1.0e+00 & 1.0e+00 & 2.5e-01 & 1.0e+00 & 4.4e-21*** & 1.8e-02* & 7.0e-02 & 7.8e-01 \\ 
\midrule \bottomrule
\end{tabular}

==> floats/texts/statisticalTests/absmax/stats-gradient-local-AbsMax.tex <==
\begin{tabular}{rllllllll}
  \toprule\midrule
 & LIME-ITEA & LIME-KR & LIME-RF & LIME-XGB & PE-ITEA & SHAP\_adj-ITEA & SHAP\_adj-KR & SHAP\_adj-RF \\ 
  \hline
  LIME-KR & 1.0e+00 &  &  &  &  &  &  &  \\ 
  LIME-RF & 1.0e+00 & 1.0e+00 &  &  &  &  &  &  \\ 
  LIME-XGB & 1.0e+00 & 1.0e+00 & 1.0e+00 &  &  &  &  &  \\ 
  PE-ITEA & 1.1e-26*** & 2.4e-26*** & 1.2e-26*** & 1.2e-26*** &  &  &  &  \\ 
  SHAP\_adj-ITEA & 1.9e-01 & 4.5e-01 & 4.4e-01 & 3.9e-01 & 9.1e-24*** &  &  &  \\ 
  SHAP\_adj-KR & 1.9e-01 & 5.0e-01 & 3.2e-01 & 3.0e-01 & 8.2e-24*** & 1.0e+00 &  &  \\ 
  SHAP\_adj-RF & 1.0e+00 & 1.0e+00 & 1.0e+00 & 1.0e+00 & 4.9e-26*** & 3.2e-01 & 3.3e-01 &  \\ 
  SHAP\_adj-XGB & 1.0e+00 & 1.0e+00 & 1.0e+00 & 1.0e+00 & 4.1e-26*** & 3.8e-01 & 4.2e-01 & 1.0e+00 \\ 
   \midrule\bottomrule
\end{tabular}

==> floats/texts/statisticalTests/absmax/stats-shap-global-AbsMax.tex <==
\begin{tabular}{rllllllll}
  \toprule\midrule
 & LIME-ITEA & LIME-KR & LIME-RF & LIME-XGB & PE\_adj-ITEA & SHAP-ITEA & SHAP-KR & SHAP-RF \\ 
  \hline
  LIME-KR & 1.0e+00 &  &  &  &  &  &  &  \\ 
  LIME-RF & 3.4e-11*** & 8.0e-11*** &  &  &  &  &  &  \\ 
  LIME-XGB & 5.3e-04*** & 8.4e-04*** & 1.0e-03** &  &  &  &  &  \\ 
  PE\_adj-ITEA & 5.6e-01 & 1.0e+00 & 1.2e-02* & 1.0e+00 &  &  &  &  \\ 
  SHAP-ITEA & 3.3e-23*** & 5.9e-24*** & 2.9e-29*** & 2.3e-27*** & 3.1e-24*** &  &  &  \\ 
  SHAP-KR & 3.0e-14*** & 4.1e-15*** & 3.9e-23*** & 5.1e-20*** & 1.8e-15*** & 6.1e-09*** &  &  \\ 
  SHAP-RF & 2.0e-06*** & 9.0e-06*** & 1.0e+00 & 4.4e-01 & 9.4e-01 & 2.2e-26*** & 1.5e-18*** &  \\ 
  SHAP-XGB & 1.0e+00 & 1.0e+00 & 6.1e-08*** & 1.0e-01 & 1.0e+00 & 2.3e-22*** & 2.5e-12*** & 2.5e-04*** \\ 
   \midrule \bottomrule
\end{tabular}

==> floats/texts/statisticalTests/absmax/stats-shap-local-AbsMax.tex <==

\begin{tabular}{rllllllll}
  \toprule \midrule
 & LIME-ITEA & LIME-KR & LIME-RF & LIME-XGB & PE\_adj-ITEA & SHAP-ITEA & SHAP-KR & SHAP-RF \\ 
  \hline
  LIME-KR & 1.0e+00 &  &  &  &  &  &  &  \\ 
  LIME-RF & 4.2e-01 & 2.1e-01 &  &  &  &  &  &  \\ 
  LIME-XGB & 1.0e+00 & 1.0e+00 & 1.0e+00 &  &  &  &  &  \\ 
  PE\_adj-ITEA & 1.4e-06*** & 1.8e-05*** & 1.0e-08*** & 2.0e-07*** &  &  &  &  \\ 
  SHAP-ITEA & 2.7e-27*** & 5.5e-27*** & 4.7e-28*** & 1.3e-27*** & 3.3e-24*** &  &  &  \\ 
  SHAP-KR & 9.5e-23*** & 3.5e-22*** & 5.7e-24*** & 2.3e-23*** & 3.0e-15*** & 2.1e-10*** &  &  \\ 
  SHAP-RF & 1.1e-06*** & 6.8e-06*** & 8.3e-10*** & 8.5e-08*** & 1.0e+00 & 1.0e-23*** & 1.4e-14*** &  \\ 
  SHAP-XGB & 7.4e-15*** & 2.9e-13*** & 6.9e-17*** & 1.2e-15*** & 2.4e-01 & 1.4e-22*** & 1.1e-11*** & 9.1e-01 \\ 
   \midrule \bottomrule
\end{tabular}

==> floats/texts/statisticalTests/exerr/stats-gradient-global-ExErr.tex <==
\begin{tabular}{rllllllll}
  \toprule\midrule
                 & LIME-ITEA & LIME-KR & LIME-RF & LIME-XGB & ME-ITEA & SHAP\_adj-ITEA & SHAP\_adjvKR & SHAP\_adj-RF \\\midrule
  LIME-KR        & 1.0e+00    &            &            &            &            &           &          &         \\ 
  LIME-RF        & 1.0e+00    & 1.0e+00    &            &            &            &           &          &         \\ 
  LIME-XGB       & 1.0e+00    & 1.0e+00    & 1.0e+00    &            &            &           &          &         \\ 
  ME-ITEA        & 7.4e-18*** & 9.3e-18*** & 3.1e-19*** & 3.2e-18*** &            &           &          &         \\ 
  SHAP\_adj-ITEA & 1.5e-02*   & 2.3e-02*   & 1.0e-04*** & 2.8e-03**  & 7.8e-12*** &           &          &         \\ 
  SHAP\_adj-KR   & 8.3e-02    & 9.2e-02    & 9.8e-04*** & 2.0e-02*   & 7.6e-13*** & 1.0e+00   &          &         \\ 
  SHAP\_adj-RF   & 1.0e+00    & 1.0e+00    & 1.0e+00    & 1.0e+00    & 1.1e-17*** & 4.2e-03** & 2.2e-02* &         \\ 
  SHAP\_adj-XGB  & 1.0e+00    & 1.0e+00    & 1.0e+00    & 1.0e+00    & 3.6e-16*** & 2.0e-01   & 6.7e-01  & 1.0e+00 \\ 
  \midrule\bottomrule
\end{tabular}

==> floats/texts/statisticalTests/exerr/stats-gradient-local-ExErr.tex <==
\begin{tabular}{rllllllll}
  \toprule\midrule
                 & LIME-ITEA & LIME-KR & LIME-RF & LIME-XGB & ME-ITEA & SHAP\_adj-ITEA & SHAP\_adj-KR & SHAP\_adj-RF \\ \midrule
  LIME-KR        & 1.0e+00    &            &            &            &            &         &         &         \\ 
  LIME-RF        & 1.0e+00    & 1.0e+00    &            &            &            &         &         &         \\ 
  LIME-XGB       & 1.0e+00    & 1.0e+00    & 1.0e+00    &            &            &         &         &         \\ 
  ME-ITEA        & 9.6e-20*** & 9.0e-20*** & 2.7e-19*** & 1.8e-19*** &            &         &         &         \\ 
  SHAP\_adj-ITEA & 2.6e-01    & 2.1e-01    & 5.6e-01    & 3.7e-01    & 1.9e-14*** &         &         &         \\ 
  SHAP\_adj-KR   & 3.2e-01    & 2.3e-01    & 6.0e-01    & 4.2e-01    & 9.4e-15*** & 1.0e+00 &         &         \\ 
  SHAP\_adj-RF   & 1.0e+00    & 1.0e+00    & 1.0e+00    & 1.0e+00    & 1.4e-16*** & 1.0e+00 & 1.0e+00 &         \\ 
  SHAP\_adj-XGB  & 1.0e+00    & 1.0e+00    & 1.0e+00    & 1.0e+00    & 6.6e-17*** & 1.0e+00 & 1.0e+00 & 1.0e+00 \\ 
  \midrule \bottomrule
\end{tabular}

==> floats/texts/statisticalTests/exerr/stats-shap-global-ExErr.tex <==
\begin{tabular}{rllll}
  \toprule \midrule
            & ME\_adj-ITEA & SHAP-ITEA  & SHAP-KR    & SHAP-RF \\ \midrule
  SHAP-ITEA & 3.9e-19***   &            &            &         \\ 
  SHAP-KR   & 5.5e-08***   & 1.3e-07*** &            &         \\ 
  SHAP-RF   & 1.0e+00      & 4.6e-21*** & 4.5e-10*** &         \\ 
  SHAP-XGB  & 1.0e+00      & 2.0e-17*** & 4.0e-06*** & 1.7e-01 \\ 
   \midrule \bottomrule
\end{tabular}


% SHAP como GT não tem: LIME, ME e SHAP_adj

==> floats/texts/statisticalTests/exerr/stats-shap-local-ExErr.tex <==
\begin{tabular}{rllll}
  \toprule \midrule
            & ME\_adj-ITEA  & SHAP-ITEA  & SHAP-KR    & SHAP-RF \\ \midrule
  SHAP-ITEA & 4.5e-18***    &            &            &         \\ 
  SHAP-KR   & 6.1e-07***    & 5.0e-08*** &            &         \\
  SHAP-RF   & 1.0e+00       & 3.2e-18*** & 6.2e-07*** &         \\ 
  SHAP-XGB  & 1.0e+00       & 8.2e-17*** & 2.2e-05*** & 1.0e+00 \\ 
  \midrule \bottomrule
\end{tabular}

% SHAP como GT não tem: LIME, ME e SHAP_adj
